Parity Objectives in Countable MDPs

We study countably infinite MDPs with parity objectives, and special cases with a bounded number of colors in the Mostowski hierarchy (including reachability, safety, Buchi and co-Buchi). In finite MDPs there always exist optimal memoryless deterministic (MD) strategies for parity objectives, but this does not generally hold for countably infinite MDPs. In particular, optimal strategies need not exist. For countable infinite MDPs, we provide a complete picture of the memory requirements of optimal (resp., $\epsilon$-optimal) strategies for all objectives in the Mostowski hierarchy. In particular, there is a strong dichotomy between two different types of objectives. For the first type, optimal strategies, if they exist, can be chosen MD, while for the second type optimal strategies require infinite memory. (I.e., for all objectives in the Mostowski hierarchy, if finite-memory randomized strategies suffice then also MD strategies suffice.) Similarly, some objectives admit $\epsilon$-optimal MD-strategies, while for others $\epsilon$-optimal strategies require infinite memory. Such a dichotomy also holds for the subclass of countably infinite MDPs that are finitely branching, though more objectives admit MD-strategies here.

==> app-coBuchi-finite-branch.tex <==

\begin{qtheorem}{\ref{thm:coBuchi}}
\thmcoBuchi
\end{qtheorem}




==> reach-buchi-inf-branch.tex <==


The following theorem is orthogonal to Theorem~7.2.7/Corollary~7.2.8
in \cite{Puterman:book}. It drops the assumption that the player's choices
are a compact subset of a complete separable metric space, but only considers
the reachability objective instead of more general objectives about a positive
bounded cumulative reward via transitions.

\begin{theorem} \label{thm:reach-eps}
MD-strategies are $\epsilon$-optimal for reachability in general MDPs.
\end{theorem}
\begin{proof}
Let $\mdp=\mdptuple$ be an MDP, and $\formula = \reach{\reachset}$ for some $\reachset \subseteq \states$.
We can assume that $\reachset = \{t\}$ for some $t \in \states$ and that $\{t\}$ is a sink.
Let $s_0 \in \states$ with $\valueof{\mdp}{s_0} > 0$, and let $\epsilon > 0$.
We show that there exists an MD-strategy~$\zstrat_\epsilon$ with $\probm_{\mdp,s_0,\zstrat_\epsilon}(\formula) \ge \valueof{\mdp}{s_0}-\epsilon$.

By the definition of the value there is an HR-strategy~$\zstrat$  such that $\probm_{\mdp,s_0,\zstrat}(\formula) \ge \valueof{\mdp}{s_0}-\frac12\epsilon$.
Defining
\[
  L = \{ w \in s_0 \states^* \mid \text{$w = s_0 s_1 \cdots s_n$ is a partial play induced by~$\zstrat$, and $s_n = t$}\}\,,
\]
we have $\probm_{\mdp,s_0,\zstrat}(L \{t\}^\omega) = \probm_{\mdp,s_0,\zstrat}(\formula) \ge \valueof{\mdp}{s_0}-\frac12\epsilon$.
Since $\states$ is countable, so is~$L$.
Hence there is a finite subset $K \subseteq L$ with $\probm_{\mdp,s_0,\zstrat}(K \{t\}^\omega) \ge \valueof{\mdp}{s_0}-\epsilon$.
Let $V \subseteq \states$ denote the states that occur in~$K$ (i.e., $V$ is the smallest set with $K \subseteq V^*$).
We have $s,t \in V$.
Since $K$ is finite, so is~$V$.

Consider the MDP~$\mdp'$ obtained from~$\mdp$ by restricting the states to $V \cup \{g\}$, where $g \not\in \states$ is a fresh state that absorbs all transitions that leave~$V$.
Since finite-state MDPs have optimal MD-strategies for reachability~\cite{Puterman:book}, there is an MD-strategy~$\zstrat_\epsilon$ on~$V$ such that $\probm_{\mdp',s_0,\zstrat_\epsilon}(\formula) \ge \probm_{\mdp',s_0,\zstrat}(\formula)$ (where we interpret~$\zstrat$ in~$\mdp'$ naturally).
Hence:
\begin{align*}
\probm_{\mdp',s_0,\zstrat_\epsilon}(\formula) 
& \ge \probm_{\mdp',s_0,\zstrat}(\formula) && \text{definition of~$\zstrat_\epsilon$} \\
& \ge \probm_{\mdp',s_0,\zstrat}(K \{t\}^\omega) && \text{$\denotationof{\formula}{s_0} \supseteq K \{t\}^\omega$} \\
&  =  \probm_{\mdp,s_0,\zstrat}(K \{t\}^\omega) && \text{all words in~$K$ are partial plays in~$\mdp'$} \\
& \ge \valueof{\mdp}{s_0}-\epsilon && \text{definition of~$K$}
\end{align*}
Extending~$\zstrat_\epsilon$ in an arbitrary way to an MD-strategy on all states in~$\states$, we obtain $\probm_{\mdp,s_0,\zstrat_\epsilon}(\formula) \ge \probm_{\mdp,s_0,\zstrat_\epsilon}(\denotationof{\formula}{s_0} \cap V^\omega) = \probm_{\mdp',s_0,\zstrat_\epsilon}(\formula) \ge \valueof{\mdp}{s_0}-\epsilon$.
\qed
\end{proof}




